Building Call Graph of WebAssembly Programs via Abstract Semantics

WebAssembly is a binary format for code that is gaining popularity thanks to its focus on portability and performance. Currently, the most common use case for WebAssembly is execution in a browser. It is also being increasingly adopted as a stand-alone application due to its portability. The binary format of WebAssembly, however, makes it prone to being used as a vehicle for malicious software. For instance, one could embed a cryptocurrency miner in code executed by a browser. As a result, there is substantial interest in developing tools for WebAssembly security verification, information flow control, and, more generally, for verifying behavioral properties such as correct API usage. In this document, we address the issue of building call graphs for WebAssembly code. This is important because having or computing a call graph is a prerequisite for most inter-procedural verification tasks. In this paper, we propose a formal solution based on the theory of Abstract Interpretation. We compare our approach to the state-of-the-art by predicting how it would perform against a set of specifically crafted benchmark programs.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
